RadAdapt: Radiology Report Summarization via Lightweight Domain Adaptation of Large Language Models

We systematically investigate lightweight strategies to adapt large language models (LLMs) for the task of radiology report summarization (RRS). Specifically, we focus on domain adaptation via pretraining (on natural language, biomedical text, or clinical text) and via discrete prompting or parameter-efficient fine-tuning. Our results consistently achieve best performance by maximally adapting to the task via pretraining on clinical text and fine-tuning on RRS examples. Importantly, this method fine-tunes a mere 0.32% of parameters throughout the model, in contrast to end-to-end fine-tuning (100% of parameters). Additionally, we study the effect of in-context examples and out-of-distribution (OOD) training before concluding with a radiologist reader study and qualitative analysis. Our findings highlight the importance of domain adaptation in RRS and provide valuable insights toward developing effective natural language processing solutions for clinical tasks.

==> figures/base_in_context.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width = .48\textwidth]{figures/base_in_context_}
    \caption{Domain adaptation via increasing number of in-context examples leads to improved performance in most models. Note this relationship does not hold for \tfive; see Section~\ref{sec:results-domain-adaptation} for discussion.}
    \label{fig:base_in_context}
\end{figure}

==> figures/base_pretrain.tex <==
\setlength{\tabcolsep}{4pt} % spacing b/w cols, default 6pt

\begin{table*}[!b]
\caption{\red{title here} Domain adaptation via pre-training on increasingly relevant data (\tfive, \scifive, \clintfivesci, \clintfive) leads to improved performance for both parameter-efficient fine-tuning methods (prefix tuning and LoRA) in most cases. This relationship is less strong for discrete prompting methods, i.e.~see Table~\ref{tab:results-base} in the appendix. Note we do not include \flantfive, whose degree of domain adaptation is difficult to rank against that of other pre-trained models. \red{todo: consider combining side-by-side w fig. 4 (parallel story) if need to cut space}}
\begin{center}
\begin{tabular}{l l | c c c c}
\textbf{Method} & \textbf{Model} & \textbf{BLEU} & \textbf{ROUGE-L} & \textbf{BERT} & \textbf{F1-Radgraph} \\
\hline
  & \tfive & 12.9 & 29.1 & 88.4 & 30.7 \\
  Prefix & \scifive & 10.3  & 28.9 & 88.4 & 30.2 \\
  tuning & \clintfivesci & \underline{11.7} & \underline{33.3} & \underline{89.3} & \underline{35.0} \\
  & \clintfive & \textbf{11.9} & \textbf{33.8} & \textbf{89.4} & \textbf{35.4} \\
\hline
\multirow{4}{*}{LoRA}   & \tfive & 13.7 & 33.9 & 89.5 & 35.2 \\
  & \scifive & \underline{13.5} &  34.6 & 89.6 & 36.1 \\
  & \clintfivesci  & 13.4  & \underline{36.4} & \underline{89.9} & \underline{37.6} \\
  & \clintfive & \textbf{14.8} & \textbf{36.8} & \textbf{89.9} & \textbf{38.2} \\
\end{tabular}
\end{center}
\label{tab:pretrain}
\end{table*}

==> figures/reader_study/table_reader_study.tex <==
\setlength{\tabcolsep}{6pt} % spacing b/w cols, default 6pt
\setlength{\extrarowheight}{1.5pt}

\begin{center}
\begin{table*}
  {tab:example}
  {\caption{sketch latex for screenshot. don't include in actual paper}}%
  {\begin{tabular}{|c|ccc|}
  \hline
  \textbf{Reader} & \textbf{Q1} & \textbf{Q2} & \textbf{Q3}\\
  \hline 
\textbf{1}      &\color{white}\colorbox{r1_Q1}{8.8 $\pm$ 2.2}
       &\color{white}\colorbox{r1_Q2}{8.8 $\pm$ 2.2}
       &\color{white}\colorbox{r1_Q3}{10. $\pm$ 0.0} \\
\textbf{2}      &\color{white}\colorbox{r0_Q1}{8.0 $\pm$ 2.5}
       &\color{white}\colorbox{r0_Q2}{8.8 $\pm$ 2.2}
       &\color{white}\colorbox{r0_Q3}{9.0 $\pm$ 2.6} \\
\textbf{3}      &\color{white}\colorbox{r2_Q1}{9.0 $\pm$ 2.1} 
       &\color{white}\colorbox{r2_Q2}{8.9 $\pm$ 2.1}
       &\color{white}\colorbox{r2_Q3}{10. $\pm$ 0.0} \\
\hline
\textbf{Pooled} &\color{white}\colorbox{r012_Q1}{8.6 $\pm$ 2.3}
       &\color{white}\colorbox{r012_Q2}{8.8 $\pm$ 2.1}
       &\color{white}\colorbox{r012_Q3}{9.7 $\pm$ 1.6} \\
  
  \hline
\end{tabular}}
\end{table*}
\end{center}
